Calibration of the photon spectrometer PHOS of the ALICE experiment

The procedure for the energy calibration of the high granularity electromagnetic calorimeter PHOS of the ALICE experiment is presented. The methods used to perform the relative gain calibration, to evaluate the geometrical alignment and the corresponding correction of the absolute energy scale, to obtain the nonlinearity correction coefficients and finally, to calculate the time-dependent calibration corrections, are discussed and illustrated by the PHOS performance in proton-proton (pp) collisions at $\sqrt{s}$ = 13 TeV. After applying all corrections, the achieved mass resolutions for $\pi^0$ and $\eta$ mesons for $p_{\rm{T}} > 1.7$ GeV/$c$ are $\sigma_m^{\pi^0} = 4.56 \pm 0.03$ MeV/$c^2$ and $\sigma_m^{\eta} = 15.3 \pm 1.0$ MeV/$c^2$, respectively.

==> MIP.tex <==
\section{Calibration using MIP peak}
\label{sec:MIP}
We performed PHOS calibration using Minimum Ionizing Particles (MIP) peak in energy spectrum.

MIP peak is hardly visible in sell energy spectrum, only clusterization helps.



In cosmic run Run 8249

\begin{figure}[h]
\unitlength\textwidth
\centering
\includegraphics[width=0.48\linewidth]{Figures/CalibMIPncell.pdf}
\hfill
\includegraphics[width=0.48\linewidth]{Figures/CalibMIPiterations1.pdf}
\caption{
\label{fig:MIP-iter} 
(Color online) Left plot: spectra of clusters with different number of cells. Right plot: cluster spectrum in PHOS before and after calibration. Width of the MIP peak is shown for each iteration.}
\end{figure}

